FENXI: Deep-learning Traffic Analytics at the Edge

Live traffic analysis at the first aggregation point in the ISP network enables the implementation of complex traffic engineering policies but is limited by the scarce processing capabilities, especially for Deep Learning (DL) based analytics. The introduction of specialized hardware accelerators i.e., Tensor Processing Unit (TPU), offers the opportunity to enhance the processing capabilities of network devices at the edge. Yet, to date, no packet processing pipeline is capable of offering DL-based analysis capabilities in the data-plane, without interfering with network operations. In this paper, we present FENXI, a system to run complex analytics by leveraging TPU. The design of FENXI decouples forwarding operations and traffic analytics which operates at different granularities i.e., packet and flow levels. We conceive two independent modules that asynchronously communicate to exchange network data and analytics results, and design data structures to extract flow level statistics without impacting per-packet processing. We prototyped and evaluated FENXI on general-purpose servers considering both adversarial and realistic network conditions. Our analysis shows that FENXI can sustain 100 Gbps line rate traffic processing requiring only limited resources, while also dynamically adapting to variable network conditions.

==> analytics.tex <==


% We implement micro-benchmark of a DL model by abstracting from the packet extraction pipeline, and feeding the hardware with jobs that are readily available from DRAM memory: so doing, we are able to preliminary select a specific accelerator hardware for the prototype, and also gather an upper bound of the full-fledged system performance.

% \subsection{DL Analytics}
% \label{related:classifier}


\subsection{Deep Learning Analytics}
\label{sec:dl}

\def\relativepower{30}
\def\relativerate{50000}
\def\relativeratek{50}

\begin{figure*}[th!]
\centering
\def\ratioFig{0.30} %size of subcaption
\def\ratioQuad{0.25}
\def\xrat{0.27} % width of figure
\def\yrat{1} % height of figure
\def\xlab{-0.2}

\pgfplotsset{
	compat=1.11,
	legend image code/.code={
		\draw[mark repeat=2,mark phase=2]
		plot coordinates {
			(0cm,0cm)
			(0.3cm,0cm)        %% default is (0.3cm,0cm)
			(0.6cm,0cm)         %% default is (0.6cm,0cm)
		};%
	}
}

\pgfplotstableread[col sep = tab]
    {Data/inference_gpu.log}
    \tableGPU

\pgfplotstableread[col sep = tab]
    {Data/inference_asc-1c-2t.log}
    \tableTPU

\pgfplotstableread[col sep = tab]
    {Data/inference_asc-4c-2t.log}
    \tableTPUtwo

\pgfplotstableread[col sep = tab]
    {Data/inference_cpu-1c.log}
    \tableCPU

\pgfplotstableread[col sep = tab]
    {Data/inference_cpu-52c.log}
    \tableCPUtwo

\subcaptionbox{Classification rate vs. batch size.\label{fig:hw_classrate}}
	[\ratioFig\textwidth] 
	{\input{Figures/hw_classrate.tex}}
\hfill%
\subcaptionbox{Batch processing and completion delay vs. batch size.\label{fig:hw_delay}}% In addition, the bold line represents the delay to complete the batch (to receive $B$ new series) for a rate of \SI{\relativeratek}{\kilo\nothing}series per second.\label{fig:hw_delay}}
	[\ratioFig\textwidth] 
	{\input{Figures/hw_delay}}
\hfill%
\subcaptionbox{Analytics vs. power relative to two targets:  \SI{\relativeratek}{\kilo class/s} and \SI{\relativepower}{\watt}.\label{fig:hw_quadrant}}
	[\ratioQuad\textwidth] 
	{\input{Figures/hw_quadrant}}
\caption{DL accelerators: throughput, delay, and power usage for various batch sizes and hardware accelerators.}
\label{fig:hw}
\end{figure*}

% \begin{figure}
% %\centering
% \includegraphics[width=0.47\textwidth]{Figures/complexity.pdf}
%   \caption{\emph{DL Analytics}: Scatter plot of model space complexity $W$ vs accuracy for different  DL models in the literature (circles: own models; star: state the art references (green stars) are included for \emph{qualitative} comparison purposes. Shapes are directly annotated with the model size and the class cardinality, and the shape radius is proportional to the model-per-class $W/K$ value. 
%   %\DR{we should simplify this figure, reducing (i) perhaps the number of models, and (ii) adding for sure the simplistic models of the literature (despite the accuracy might be not known}}\afnote{probably repurpose the figure to talk about latency/resource usage because model complexity it's pretty opaque. It might turn out that at this scale, the model size is still too small to have an actual impact on inference latency.
%   }
%     \label{fig:analytics-complexity}
% \end{figure}

We observe a dichotomy in the \gls{dl} models that the scientific community has designed for network traffic processing. On the one hand, some models target the accuracy of the task, but ignore system requirements. Such models can contain millions of weights~\cite{chen2017bigdata}. On the other hand, the work considering system constraints adopts a simplistic view of \gls{dl} models, \eg{} the model in Taurus~\cite{swamy2020taurus} uses two-digit weights. We therefore consider reasonably sized models (\eg{} \SI{90}{\kilo\nothing} weights, which amount to \SI{200}{\kilo B} with floating point \num{32} precision), which can identify hundreds of applications and is trained with state-of-the-art machine learning frameworks (\ie{} Tensorflow) using real traffic traces. We disregard model training and accuracy, which are out of the scope of this paper. Rather, our focus is on accelerating the execution of such models in the data plane.

Since the model size is orders of magnitude smaller than typical \gls{cnn} models used for image processing, a CPU has the capacity to execute \gls{dl} inference (which would avoid round-trips to the offloading hardware), but running the \gls{dl} model on dedicated processors can bring benefits with respect to power usage, throughput, and latency. As such, we need to preliminary benchmark these candidate choices to decide if the prototype should delegate DL model inference to GPU/TPU or run it in the general purpose CPU. 

% \begin{figure}[t!]
% 	\centering
% 	\includegraphics[width=0.48\textwidth]{Figures/DL-hardware-micro-benchmark.png}
% % 	\input{Figures/classrate.tex}
% 	%\includegraphics[width=0.3\textwidth]{Figures/performance-comparison.pdf}
% 	%includegraphics[width=0.42\textwidth]{Figures/power-comparison.pdf}
% 	\caption{\emph{DL accelerators}: Classifications rate for  different batching size (x-axis) and configuration of CPU, GPU and TPUs. \DR{equivalent delay on top?}}
% 	\label{fig:hw}
% \end{figure}


% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\textwidth]{Figures/quadrant-class}
%     \caption{\emph{DL accelerators}: Scatter plot of throughput vs power budget across different CPU, GPU and TPU configurations. \DR{Conclusions: a signle batch size is not enough. All figures have a different look and feel, we should make it homogeneous}}
%     \label{fig:hw-scatter}
% \end{figure}

We run preliminary experiments on servers equipped with Intel Xeon Platinum 8164 CPUs  @ 2.00GHz (L1/L2/L3 caches 32 data+32 instruction)/1024/36608 kB) and 100 Gbps Mellanox MCX515A-CCAT ConnectX-5. As \gls{dl} offload hardware, we use either an Huawei Atlas 300 TPU (equipped with \num{4}$\times$ Ascend 310 chips), or an Nvidia V100 GPU. To provide a fair comparison across the TPU and GPU cases, we do not employ the native Huawei Mind Studio stack and rather  cross-compile the original TensorFlow model for the Huawei Atlas engine. We now review performance in terms of analytics throughput, delay, and power consumption varying the number of series or which inference is run in parallel \ie{} batch sizes $B$. Results are shown in \Cref{fig:hw}.

\paragraph{Throughput and Latency} We report analytics throughput in \Cref{fig:hw_classrate} in terms of classification per second achieved by CPU (either 1 or 52 cores), GPU, and TPU (either 1 or 4 cores). Whereas CPU and GPU are optimized for large batch size $B$, the TPU process analytics faster for small size $B$. 

We then report in \Cref{fig:hw_delay} the maximum delay between the time at which the NIC receives the \ith{K} packet of a flow and the time it gets the flow label. We distinguish here between the \emph{batch completion delay}, which is the time needed for a flow to wait for the other $B-1$ flows to arrive, and the \emph{batch inference delay}, which is the time needed for the result of the batch to be available. To simplify our calculation, we used \SI{50}{\kilo class/s} as the constant flow arrival rate. The batch completion delay is dominant in the delay. As a consequence, setting the batch size is key: a large batch results in a long delay, while a small batch leads the inference system to run in a sub-optimal operational regime.

%ore generally we should stick to batches smaller or equal than \num{512} to prevent both the ratio of untagged packet in elephant flows and the ratio of post-mortem analytics of short-lived flows to incresae.

% The demonstration reveals that large batch size $B\approx$\DR{XXX} 
% to be  impractical due to the latency introduced by batch completion: while a flow waits for the other $B-1$ flows to arrive, new arriving packets remain untagged, and worse, some mice flow may be classified \emph{post-mortem}. 

% With regards to our requirements on delays (see \Cref{sec:requirements}), we should opt for offloading small batch sizes to TPU, 
% at the price of lower throughput processing, saturating to about \SI{200}{\kilo\nothing} jobs per second according to our measures. From \Cref{tab:dataset}, such an analytics throughput corresponds to a traffic at multi-hundred gigabits per second. 

\paragraph{Power Usage}
\Cref{fig:hw_quadrant}, illustrates
the tradeoff of analytics throughput versus power usage for varying batch sizes as a scatter plot of the power  ($x$-axis) and classification rate ($y$-axis) normalized with respect to reference values of \SI{\relativepower}{\watt} and \SI{\relativeratek}{\kilo class/s}.  The top-left square highlights desirable configurations although the bottom-right one includes operational regions that should be avoided.  For instance, only one hardware configuration (TPU with \num{1} core) with a couple of settings can meet the requirement of our configuration (\SI{\relativepower}{\watt} and \SI{\relativeratek}{\kilo class/s}), while the other hardware configurations fail in at least one dimension.

From \Cref{fig:hw_quadrant}, we conclude that CPU does not offer a viable hardware platform for fast analytics since the energy consumption is too large while it does not offer processing gains. TPU offers a more energy efficient alternative, especially with regards to its higher processing performance for small batches, while GPU is the option to cope with large throughput requirements. %However it may not be able to sustain very high throughput.

%It also follows that no single-batch size can achieve both fast operation at low load, as well as high throughput at high load -- for which variable batch size is a necessary system component.

==> context.tex <==
\section{Context}
To ease the reading of the paper, we consider a given network analytics, namely a traffic classifier, as an example. \acrshort{fix} can however apply on many other analytics and we try, as often as possible, to generalize our conclusions. We chose a traffic classifier, because $(i)$ it is a classic network analytics operation that can be done after a few packets~\cite{teixeira06ccr}; and $(ii)$ recent studies have demonstrated significant increase of the classifier performance when using \gls{dl} approaches~\cite{AcetoCMP19}. The traffic classifier that we consider here provides a strong motivation for the implementation of \acrshort{fix} since it can classify flows across \num{200} applications, which is at least twice more applications than previous known analytics~\cite{AcetoCMP19}.


%\acrshort{fix} aims at augmenting the features exported by a network device by analyzing its data plane traffic with \gls{dl} models. 
We focus on Internet traffic by extracting IP \emph{packets} and by analyzing network \emph{flows}, as identified by the \num{5}-tuple at the network layer (IP addresses and ports of both source and destination plus protocol). With \emph{early application identification}~\cite{crotti07ccr,teixeira06ccr} (\ie{} classification), \acrshort{fix} triggers the analytics at the \ith{K} packet of each flow, though for other analytics \acrshort{fix} can exploit any flow subset. For the sake of clarity, we stick to the implementation of analytics after the \ith{K} packet of each flow in the following of the paper, and by default $K$ is equal to \num{10}, which corresponds to a trade-off between the amount of  information to analyze and the delay to process the analytics~\cite{pandorabox}. Formally we extract from each flow a \emph{series} $s$ containing $K$ information, which are extracted from the $K$ first packets $s = \{s_1, \dots, s_K\}$ of the flow. We denote by $S_K$ the set of series of size $K$. In the case of traffic classification~\cite{pandorabox}, the information $s_i$ extracted from the \ith{i} packet of a flow contains packet length and direction. Other analytics may require information such as \gls{iad}~\cite{AcetoCMP19}.

To better understand the requirements and complex dynamics involved in the \acrshort{fix} system we first explore the traffic characteristics observing real world scenario and deep learning analytics with the objective of defining our system requirements.

\input{traffic.tex}

\input{analytics.tex}



==> traffic.tex <==
\begin{figure*}[th!]
\def\ratio{0.32}
\def\yrat{1}
\def\xrat{0.23}
\centering
%%%%%%%%%%%%%%%%%%%% FIGURE cdf nb of packets per flow
% % \subcaptionbox{\gls{cdf} of the number of packets per flow. The flow are TCP flows extracted in the datasets. We omit both initial SYN and ACK packets.\label{fig:cdf}}
% % 	[\ratio\textwidth] 
% % 	{\input{Figures/cdf_pkts_per_flow.tex}}
%%%%%%%%%%%%%%%%%% Figure Bursts choice CDF 1
% \subcaptionbox{Burst: The ratio between maximum and minimum \gls{iad} in \SI{200}{\milli\second} time interval.  
%     \label{fig:bursts}}
%     [\ratio\textwidth]
%     {\input{Figures/cdf_bursts_isd.tex}}%bursts.csv
% \hfill%
%%%%%%%%%%%%%%%% Figure Burst choice CDF 2
% \subcaptionbox{
% We measured the number of new series arrived in \SI{150}{\milli\second} intervals. Then we computed the ratio between the max and the min series arrival within the same second.
% %  On the $y$-axis, the ratio max to min in boxplot (max, \ith{75}, \ith{25}, and min percentiles).
%     \label{fig:bursts}}
%     [\ratio\textwidth]
%     {\input{Figures/cdf_bursts.tex}}%bursts.csv
%%%%%%%%%%%%%%%%%%%%%
\subcaptionbox{Delays: Ratio of dead short-lived flows after the \ith{10} packet.\label{fig:dead}}
	[\ratio\textwidth]
	{\input{Figures/dead_flows.tex}}
\hfill%
\subcaptionbox{Delays: Number of received packets for long-lived flows after the \ith{10} packet.\label{fig:shift}}
	[\ratio\textwidth]
	{\input{Figures/pkts_per_shift.tex}}
\hfill%
	%%%%%%%%%%%%%%%% Figure Burst Choice boxplot batch completion
\subcaptionbox{Burst: The ratio between the max and the min series arrival rate between 6 consecutive \SI{150}{\milli\second} slots.
%Bursts: We measured batch completion delays during \SI{10}{\minute}. We show the distribution of per-second ratio of longest/shortest delays.
    \label{fig:bursts}}
    [\ratio\textwidth]
    {\input{Figures/cdf_bursts}}%bursts.csv
%%%%%%%%%%%%%%%%%%%%%%
\caption{Dataset analysis regarding bursts of series arrival rate and delays. Boxplots show \ith{99}, \ith{75}, \ith{25}, and $1^{\text{st}}$ percentiles.}
\end{figure*}

\subsection{Traffic Characteristics}
\label{sec:requirements}

%We design \acrshort{fix} to be implemented in any device in the Internet, for example a router in an enterprise campus, in an area optical access, and transit to \gls{isp}. 
To estimate the requirements and the performance that \acrshort{fix} needs to achieve, we studied traffic characteristics extracted from three datasets. Two datasets (\textit{campus} and \textit{access}) are private datasets that we obtained from an operator in China. The third dataset (\textit{transit}) comes from the public \gls{mawi} project\footnote{\url{http://mawi.wide.ad.jp/} -- extracted 2020-02-12, 2020-03-04, 2020-03-25, 2020-04-08, 2020-05-27, 2020-06-03, 2020-06-10} so that our results can be reproduced. In each dataset, we identified the flows, %by means of the classic IP \num{5}-tuple, 
from which we extracted packet time-stamps and lengths. We derive the following requirements for \acrshort{fix}.

\paragraph{Throughput}
We show in \Cref{tab:dataset} the total number of packets, flows and series (\ie{} flows with more than ten packets) in the dataset. We use datasets' traffic characteristics to derive the required performance in terms of packet (\ie{} Mpps) and series processing speed (\ie{} class./s) for a \SI{100}{\giga{}bps} linecard at maximum load. We conclude that a single \SI{100}{\giga{}bps} linecard should be able to sustain on average \SI{15}{Mpps} and \SI{50}{kclass/s}. 

\begin{table}[h]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{@{}cccccccc}
        \toprule
         & \multicolumn{4}{c}{\textbf{Traffic characteristics}} & \multicolumn{3}{c}{\textbf{ Rate at 100 {Gbps}}}
         \\ \cmidrule(l){2-5} \cmidrule(l){6-8}
         \textbf{dataset} & \textbf{vol.} & \textbf{\#{}pkts} & \textbf{\#{}flows} & \textbf{\#{}series}  & \textbf{packet} & \textbf{flow} & \textbf{series}
         \\ & [\SI{}{\giga B]} &  [\SI{}{\mega\nothing]} & %\textbf{\#{}serie}
         [\SI{}{\kilo\nothing]} & [\SI{}{\kilo\nothing]} & 
         [\SI{}{\mega pps}]& [\SI{}{\kilo flows/s}] & [\SI{}{\kilo class/s}]
         \\ \midrule 
%%%%
access & \num{765} & \num{858}
    & \num{3963} & \num{2481}
    & \num{14.0} & \num{64.7} & \num{40.5} \\
transit & \num{870} & \num{923}
    & \num{2476} & \num{1968}
    & \num{13.2} & \num{35.5} & \num{28.3} \\
campus & \num{483} & \num{516}
    & \num{2700} & \num{1718}
    & \num{13.3} & \num{69.8} & \num{44.4} \\
%%%%
         \bottomrule
    \end{tabular}
    \caption{Traffic characteristics in real datasets.}
    \label{tab:dataset}
\end{table}

% Previous ver.
%We show in \Cref{tab:dataset} the number of packets, flows and series (\ie{} flows with more than ten packets). The bottleneck in \acrshort{fix} can come from the \gls{nic} (too large throughput), from the packet processing (too many packets per second), from the flow storage (too many flows per second), or from the hardware accelerator (too many series per second). As in \Cref{fig:hw}, we use the reference of \num{50}{\kilo{}series/s} for the classification rate of the hardware accelerator and we provide in \Cref{tab:dataset} the equivalent rate as bits, packets, and flows as observed in our datasets. This reference classification rate can sustain in average the traffic rate of a  \num{100}{\giga{}bps} router.   

% \begin{table}[h]
%     \centering
%     \scriptsize
%     \setlength{\tabcolsep}{4pt}
%     \begin{tabular}{@{}llllllll}
%         \toprule
%          & \multicolumn{4}{c}{\textbf{Global Numbers}} & \multicolumn{3}{c}{\textbf{Relative to \SI{50}{kclass/s}}}
%          \\ \cmidrule(l){2-5} \cmidrule(l){6-8}
%          \textbf{dataset} & \textbf{vol.} & \textbf{\#{}pkts} & \textbf{\#{}flows} & \textbf{\#{}series} & \textbf{Through.} & \textbf{packet} & \textbf{flow}
%          \\ \midrule 
% %%%%
% access & \SI{765}{\giga B} & \SI{858}{\mega\nothing}
%     & \SI{3963}{\kilo\nothing} & \SI{2481}{\kilo\nothing}
%     & \SI{121}{\giga bps} & \SI{17.3}{Mpps} & \SI{80}{kflows/s} \\
% transit & \SI{870}{\giga B} & \SI{923}{\mega\nothing}
%     & \SI{2476}{\kilo\nothing} & \SI{1968}{\kilo\nothing}
%     & \SI{178}{\giga bps} & \SI{23.4}{Mpps} & \SI{63}{kflows/s} \\
% campus & \SI{483}{\giga B} & \SI{516}{\mega\nothing}
%     & \SI{2700}{\kilo\nothing} & \SI{1718}{\kilo\nothing}
%     & \SI{116}{\giga bps} & \SI{15.0}{Mpps} & \SI{79}{kflows/s} \\
% %%%%
%          \bottomrule
%     \end{tabular}
%     \caption{Traffic characteristics in real datasets.}
%     \label{tab:dataset}
% \end{table}

\paragraph{Delays} Flows can be classified in \emph{short-lived} and \emph{long-lived}. The former represent the vast majority of the flows while the latter are responsible of the vast majority of data volume. In our datasets, considering the target of analytics after the \ith{10} packet we identify a flow as short-lived if it has less than 35 packets, long-lived otherwise. \acrshort{fix} targets to infer a series for a short-lived flow before its end to prevent \emph{post-mortem} analytics. However, the life expectation of short-lived flows after the \ith{10} packet arrival ranges from a few milliseconds to minutes (see \Cref{fig:dead}). \acrshort{fix} also targets to tag packets of long-lived flows as soon as possible to 
enable traffic differentiation~\cite{LiNCGM19}. But the \gls{iad} of packets is also widely distributed (see \Cref{fig:shift}). We conclude that a delay requirement cannot be strictly and universally set, since it also depends on the location of the device in the network (see the differences between datasets). Yet, a target in the range of \SIrange{10}{30}{\milli\second} enables a low fraction of both untagged packets and post-mortem analytics.

\paragraph{Burst} Network traffic is subject to instantaneous high-load over a short period, \ie{} bursts~\cite{JinGXSNLQW19}, which also reflect in the arrival rate of series. 
From \SI{10}{\minute} of each dataset, we measured the number of new series arrived in \SI{150}{\milli\second} intervals and plot the ratio between the maximum and the minimum values registered over 6 \SI{150}{\milli\second} slots. 
% the \gls{iad} between consecutive \emph{series} (\ie{} flow reaching the \ith{10} packet).
%number of new series arrived in intervals of \SI{150}{\milli\second} 
%the delays to  build consecutive batches of new series, 
%To show the impact of bursts into batch completion time, we computed the ratio between the longest and the shortest completion delays observed within the same second.  
%and then, every second, we compute the ratio between the maximum and minimum \glspl{iad}. 
%per-interval series arrival.
%delays. 
A high ratio indicates that the series arrival rate is subject to a high variation within the same second. Results in \Cref{fig:bursts} show that series arrival rate can vary a lot \ie{} from 2 up to 5 times. Hence \acrshort{fix} should be able to absorb bursts by dynamically adapting to network conditions with the twofold objective of improving analytics processing (see \Cref{sec:dl}) efficiency and reducing the time required to obtain analytics result \ie{} avoid waiting in case of limited load.
%such that %, within the same second, %the \gls{iad} varies by two to five orders of magnitude. 
%%the arrival rates vary by a factor of at least two in the majority of time.  
%a given batch of eight series can be completed two orders of magnitude faster than another batch in the same second.

%We also conceived a synthetic dataset to get a wide diversity of network configurations and to stress the \acrshort{fix} system in extreme conditions. We implemented a program that creates new flows of packet following a Poisson distribution for various flow arrival rate. To stick to realistic traffic, we re-used the packet trains of the flows that we extracted from the real traces to create the traffic flow in our synthetic traces. Each created new flow has a randomized IP address and port, but the number of packets, the length of each packet, and the \gls{iad} between packets are randomly chosen in the catalog of real extracted flows. This program generates traces with any flow arrival rate.






==> trashed_cache.tex <==

\subsection{Analysis (Long version)}

\gsnote{This whole subsection is optional}

Let $\sigma \in S_\delta$ be a prefix of size $\delta$. Let $D(\sigma)$ be the set of series in $S_K$ that have $\sigma$ as prefix $
D(\sigma) = \{s \in S_K: q_\delta(s) = \sigma\}$

We distinguish four types of prefixes, as represented in \Cref{fig:prefix}. A prefix $\sigma \in S_\delta$ is \emph{non-profitable} if $D(\sigma)$ contains only one series. Such a prefix does not improve the performance of the cache. Among the profitable prefixes, we then distinguish the \emph{safe} and the \emph{dangerous} prefixes. A safe prefix is a prefix such that multiple series in $S_K$ share it and all these series have the same label. The hit generated by a safe prefix is a good hit. On the contrary, a dangerous prefix generates a hit for series in $S_K$ that have different labels. 
% $$
% |D(\sigma)| > 1\hspace{0.7em} \&\hspace{0.7em} \exists (s, s')\in D(\sigma)\times D(\sigma): f(s) \neq f(s')
% $$
% $$
% |D(\sigma)| > 1\hspace{0.7em} \&\hspace{0.7em} \forall(s,s') \in D(\sigma)\times D(\sigma), f(s) = f(s')
% $$

\begin{figure}[ht]
\centering
\input{Figures/prefix.tex}
\caption{Typology of prefixes of size $\delta = 2$ for series in $S_5$.} \label{fig:prefix}
\end{figure}



The hit generated by a dangerous prefix is either a good or an error hit, but some prefixes are more dangerous than others. We say that a prefix $\sigma$ is \emph{toxic} when the most popular label among all \emph{flows} with series in $D(\sigma)$ represents less than a given threshold $\beta$ of the total number of flows. We set $\beta = \num{0.7}$.  
%Formally:
% \begin{align*}
% |D(\sigma)| > 1 \hspace{2pt} & \& \hspace{2pt} \exists (s, s')\in D(\sigma)\times D(\sigma): f(s) \neq f(s') \\
% & \& \hspace{2pt} \frac{\max_{f \in \mathcal L}\left\{\sum_{s \in D(\sigma):f(s)=f}p_s\right\}}
% {\sum_{f \in \mathcal L}\left\{\sum_{s \in D(\sigma):f(s)=f}p_s\right\}} \leq \beta
% \end{align*}
The hit generated by a toxic prefix has a high risk of being an error hit.


\begin{figure*}
\def\ratio{0.32}
\def\rat{0.25}
\def\yrat{0.85}
\def\widthbar{10pt}
\centering
\subcaptionbox{Neglecting popularity skew\label{fig:danger}}
	[\ratio\textwidth] 
	{\input{Figures/danger_ratio.tex}}
\hfill%
\subcaptionbox{Application-granularity, real  popularity.\label{fig:danger_queries}}
	[\ratio\textwidth]
	{\input{Figures/danger_queries.tex}}
\hfill%
\subcaptionbox{Category-granularity,   real popularity\label{fig:danger_queries_cat}}
	[\ratio\textwidth]
	{\input{Figures/danger_queries_cat.tex}}
\caption{Ratio of prefixes of a given size ($x$-axis) and distribution of non-profitable, safe, and dangerous prefixes.}\label{fig:pref}
\end{figure*}

We studied the distribution of non-profitable, safe, dangerous, and toxic prefixes in the traffic. We used the labels obtained from our \gls{dl} per-application and per-categories classifier on  \num{\nbseries}k series in $S_{10}$ in the \emph{campus} dataset. 
We present the results in \Cref{fig:pref}.

When studying the distribution on series without taking into account their respective popularity (\Cref{fig:danger}), the cache designer may be disappointed since most prefixes are non-profitable. However, when taking into account their respective popularity (see \Cref{fig:danger_queries} and \Cref{fig:danger_queries_cat}), a large majority of flows have profitable prefixes, so the gain in hit-ratio is likely to increase. Furthermore, the ratio of flows that have toxic prefixes is insignificant. A large majority of flows (\SI{97.1}{\percent} for prefix $\delta = 3$) are either safe hits or hits with a probability greater than \num{0.7} to be good. The error is thus expected to stay limited.


